Multi-level analysis of compiler induced variability and performance tradeoffs

Successful HPC software applications are long-lived. When ported across machines and their compilers, these applications often produce different numerical results, many of which are unacceptable. Such variability is also a concern while optimizing the code more aggressively to gain performance. Efficient tools that help locate the program units (files and functions) within which most of the variability occurs are badly needed, both to plan for code ports and to root-cause errors due to variability when they happen in the field. In this work, we offer an enhanced version of the open-source testing framework FLiT to serve these roles. Key new features of FLiT include a suite of bisection algorithms that help locate the root causes of variability. Another added feature allows an analysis of the tradeoffs between performance and the degree of variability. Our new contributions also include a collection of case studies. Results on the MFEM finite-element library include variability/performance tradeoffs, and the identification of a (hitherto unknown) abnormal level of result-variability even under mild compiler optimizations. Results from studying the Laghos proxy application include identifying a significantly divergent floating-point result-variability and successful root-causing down to the problematic function over as little as 14 program executions. Finally, in an evaluation of 4,376 controlled injections of floating-point perturbations on the LULESH proxy application, we showed that the FLiT framework has 100 precision and recall in discovering the file and function locations of the injections all within an average of only 15 program executions.

==> Makefile <==
TOPLEVEL   := bisect.tex
TARGET     := bisect.pdf
DIFF_TARGET:= diff.pdf
TARGETS    := $(TARGET)
TARGETS    += $(DIFF_TARGET)
GREY_TARGETS:= $(TARGETS:%.pdf=%-grey.pdf)
COPY_TARGETS:= $(TARGETS:%.pdf=%-copy.pdf)
ZIP_TARGET := 2019-hpdc.zip
ZIP_DIR    := $(basename $(ZIP_TARGET))

DEPFILES   :=
DEPFILES   += $(wildcard *.cls)
DEPFILES   += $(wildcard *.bib)
DEPFILES   += $(wildcard *.bst)
DEPFILES   += $(wildcard inputs/*.tex)
DEPFILES   += $(wildcard inputs/algorithms/*.tex)
DEPFILES   += $(wildcard inputs/figures/*.tex)
DEPFILES   += $(wildcard inputs/tables/*.tex)
DEPFILES   += $(wildcard inputs/notes/*.tex)
DEPFILES   += $(wildcard images/*.pdf)
DEPFILES   += $(wildcard images/timing/*.pdf)
DEPFILES   += $(TOPLEVEL)
DEPFILES   += Makefile

GARBAGE    :=
GARBAGE    += comment.cut
GARBAGE    += $(TOPLEVEL:%.tex=%.log)
GARBAGE    += $(TOPLEVEL:%.tex=%.out)
GARBAGE    += $(TOPLEVEL:%.tex=%.aux)
GARBAGE    += $(TOPLEVEL:%.tex=%.dvi)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb)
GARBAGE    += $(TOPLEVEL:%.tex=%.cb2)
GARBAGE    += $(TOPLEVEL:%.tex=%.bbl)
GARBAGE    += $(TOPLEVEL:%.tex=%.blg)
GARBAGE    += $(TOPLEVEL:%.tex=%.tdo)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.in)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.lua)
GARBAGE    += $(TOPLEVEL:%.tex=%.markdown.out)
GARBAGE    += $(addprefix _markdown_,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(addprefix _minted-,$(TOPLEVEL:%.tex=%))
GARBAGE    += $(wildcard figures/*-eps-converted-to.pdf)

# To use custom fonts, build with xelatex instead
LATEX      := pdflatex
LATEX      += -shell-escape
#LATEX       = xelatex
LATEXDIFF  := latexdiff --exclude-textcmd="section,subsection"

.PHONY: default
default: $(TARGET) $(TARGET:%.pdf=%-copy.pdf) $(TARGET:%.pdf=%-grey.pdf)

.PHONY: all
all: $(TARGETS) $(COPY_TARGETS) $(GREY_TARGETS) $(ZIP_TARGET)

$(TARGET): $(DEPFILES)

%.pdf: %.tex
	@echo "$< -> $@"
	@$(LATEX) $< </dev/null >/dev/null || (tail -n 30 $*.log && false)
	@-bibtex $*  </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null
	@$(LATEX) $< </dev/null >/dev/null

%-copy.pdf: %.pdf
	@echo "$< -> $@"
	@cp $< $@

%-grey.pdf: %.pdf
	@echo "$< -> $@"
	@gs \
	  -sOutputFile="$@" \
	  -sDEVICE=pdfwrite \
	  -sColorConversionStrategy=Gray \
	  -dProcessColorModel=/DeviceGray \
	  -dCompatibilityLevel=1.4 \
	  -dNOPAUSE \
	  -dBATCH \
	  -q \
	  "$<"

images/%.eps: images/%.dot
	dot $< -Tps -o $@

images/%.ps: images/%.tex
	@echo "$< -> $@"
	@(cd images && $(LATEX) $(notdir $<)) </dev/null >/dev/null \
		|| (tail -n 30 $(<:%.tex=%.log) && false)

.PHONY: diff
diff: diff.pdf

diff.tex: old.tex new.tex
	@echo "old.tex + new.tex -> $@"
	@$(LATEXDIFF) old.tex new.tex 2>/dev/null > diff.tex

new.tex: latexpand $(DEPFILES)
	@echo "bisect.tex -> new.tex"
	@./latexpand --fatal --verbose --output new.tex bisect.tex 2>/dev/null

GARBAGE    += new.tex
GARBAGE    += diff.tex
TARGETS    += diff.pdf
GARBAGE    += old.log
GARBAGE    += old.out
GARBAGE    += old.aux
GARBAGE    += old.dvi
GARBAGE    += old.cb
GARBAGE    += old.cb2
GARBAGE    += old.bbl
GARBAGE    += old.blg
GARBAGE    += old.tdo
GARBAGE    += old.markdown.in
GARBAGE    += old.markdown.lua
GARBAGE    += old.markdown.out
GARBAGE    += old.pdf
GARBAGE    += new.log
GARBAGE    += new.out
GARBAGE    += new.aux
GARBAGE    += new.dvi
GARBAGE    += new.cb
GARBAGE    += new.cb2
GARBAGE    += new.bbl
GARBAGE    += new.blg
GARBAGE    += new.tdo
GARBAGE    += new.markdown.in
GARBAGE    += new.markdown.lua
GARBAGE    += new.markdown.out
GARBAGE    += new.pdf
GARBAGE    += new.tex
GARBAGE    += diff.log
GARBAGE    += diff.out
GARBAGE    += diff.aux
GARBAGE    += diff.dvi
GARBAGE    += diff.cb
GARBAGE    += diff.cb2
GARBAGE    += diff.bbl
GARBAGE    += diff.blg
GARBAGE    += diff.tdo
GARBAGE    += diff.markdown.in
GARBAGE    += diff.markdown.lua
GARBAGE    += diff.markdown.out
GARBAGE    += diff.tex

.PHONY: clean
clean:
	rm -rf $(GARBAGE)

.PHONY: veryclean
veryclean: clean
	rm -f $(TARGETS)
	rm -f $(COPY_TARGETS)
	rm -f $(GREY_TARGETS)
	rm -rf $(ZIP_DIR)
	rm -f $(ZIP_TARGET)

.PHONY: distclean
distclean: veryclean

.PHONY: zip
zip: $(ZIP_TARGET)

$(ZIP_DIR):
	mkdir -p $(ZIP_DIR)

# @param 1: source file
# @param 2: destination directory
define COPY_TO_PATH
	mkdir -p $(strip $2)/$(strip $(dir $1))
	cp $1 $2/$1
	
endef

$(ZIP_TARGET): $(DEPFILES) | $(ZIP_DIR)
	$(foreach f,$(DEPFILES),$(call COPY_TO_PATH,$f,$(ZIP_DIR)))
	zip -r $(ZIP_TARGET) $(ZIP_DIR)

